Enhancing Zero-shot Audio Classification using Sound Attribute Knowledge from Large Language Models

Zero-shot audio classification aims to recognize and classify a sound class that the model has never seen during training. This paper presents a novel approach for zero-shot audio classification using automatically generated sound attribute descriptions. We propose a list of sound attributes and leverage large language model's domain knowledge to generate detailed attribute descriptions for each class. In contrast to previous works that primarily relied on class labels or simple descriptions, our method focuses on multi-dimensional innate auditory attributes, capturing different characteristics of sound classes. Additionally, we incorporate a contrastive learning approach to enhance zero-shot learning from textual labels. We validate the effectiveness of our method on VGGSound and AudioSet\footnote{The code is available at \url{https://www.github.com/wsntxxn/AttrEnhZsAc}.}. Our results demonstrate a substantial improvement in zero-shot classification accuracy. Ablation results show robust performance enhancement, regardless of the model architecture.

==> rebuttal.tex <==
We would like to clarify misunderstandings of our work:

1. R#3 and R#8 think we miss the comparison with audio-text models such as CLAP and Pengi.
This is a significant misunderstanding.
Nowadays "zero-shot audio classification" often refers to the setting of CLAP: the model is trained on audio-text data but not exposed to the evaluation classification dataset (e.g., ESC50).
In this setting, models are likely to have been exposed to audio-text pairs with target classes during training.
For instance, the model has encountered the "[dog barking](audio)-[a dog barks](text)" pair so it can recognize the dog barking sound in ESC50.
Our model tackles a more challenging scenario where audio samples and class labels are entirely unseen during training.
For example, for the Minions voice, CLAP would struggle with accurate classification because the text "Minions" itself does not contain any descriptive information about sound characteristics.
However, if we describe the attributes, such as the Minions' voice being brief and high-pitched, resembling children sound, the model might be able to classify it.
This has been emphasized in the fourth paragraph of Introduction.

Since previous audio-text models only use text descriptions like "sound of xx", applying such contrastive learning methods is just the same as our baseline: using "class (& definition)" as the text label.
Therefore, our comparison is fair.

2. R#3 questions the novelty of our method compared with WavCaps, which also employs LLM for generating or improving text descriptions of audio.
We do not think the problem of improving descriptions using LLMs for audio-text learning has been solved and disagree that exploration on this point is not novel.
As pointed above, such descriptions are not optimal.
The attribute set itself is a contribution and our method can also be used to augment CLAP training data.

% WavCaps reformatted classification labels or user-uploaded descriptions into "sound of xx".
% As pointed above, such descriptions do not leverage sound attributes for distinguishing sounds.
% Therefore, our novelty is not trivial.
% The attribute set itself is a contribution and our method can also be used to augment CLAP training data, which we leave for future work. 

3. R#9 has concern about the clarity.
However, we have detailed the methods used to achieve a balanced distribution across fold splits, which is the most crucial pre-processing step.
Additionally, dataset sizes and experimental setups have been explained in Section 4.
Therefore, the clarity is underestimated.
%I don't think the last part clarity needs rebuttal, see word limit and consider cutting down this part. If we still have space, add a paragraph stressing the novelty of the paper, that this knowledge-enhanced method can be further added to LLM training. The attribute set itself is the final product and ample experiments show that they are effective in solving an important problem, which is acoustic classification on unseen sounds. 

